Achieving High Coverage for Floating-point Code via Unconstrained Programming (Extended Version)

Achieving high code coverage is essential in testing, which gives us confidence in code quality. Testing floating-point code usually requires painstaking efforts in handling floating-point constraints, e.g., in symbolic execution. This paper turns the challenge of testing floating-point code into the opportunity of applying unconstrained programming --- the mathematical solution for calculating function minimum points over the entire search space. Our core insight is to derive a representing function from the floating-point program, any of whose minimum points is a test input guaranteed to exercise a new branch of the tested program. This guarantee allows us to achieve high coverage of the floating-point program by repeatedly minimizing the representing function. We have realized this approach in a tool called CoverMe and conducted an extensive evaluation of it on Sun's C math library. Our evaluation results show that CoverMe achieves, on average, 90.8% branch coverage in 6.9 seconds, drastically outperforming our compared tools: (1) Random testing, (2) AFL, a highly optimized, robust fuzzer released by Google, and (3) Austin, a state-of-the-art coverage-based testing tool designed to support floating-point code.

==> mcmc.tex <==
  Monte Carlo Markov Chain (MCMC)
 sampling is a stochastic  global optimization
 algorithm. 
A fundamental fact regarding MCMC is
 that it follows the target distribution asymptotically.  Below, we give the results~\cite{DBLP:dblp_journals/ml/AndrieuFDJ03}  with the discrete-valued probability.
\begin{lem}
  Let $x$ be a random variable, $A$ be an  enumerable set of the
  possible values of $x$. Let $f$ be a target probability  distribution for $x$, \ie,  the probability of $x$ taking value  $a$ is  $f(a)$.  Then, for an MCMC sampling sequence
  $x_1,\ldots,x_n\ldots$ and a probability density function
  $P(x_n=a)$ for each $x_n$, we have $P(x_n =a) \rightarrow f(a)$.
\label{lem:pdf}
\end{lem}
 
For example, consider the target distribution of coin tossing with
$0.5$ probability for having the head. An MCMC sampling is a sequence
of random variables $x_1$,\ldots, $x_n,\ldots$, such that the probability of
$x_n$ being ``head'', denoted by $P_n$, converges to $0.5$. 


